Get In Video: Add Anything You Want to the Video

Video editing increasingly demands the ability to incorporate specific real-world instances into existing footage, yet current approaches fundamentally fail to capture the unique visual characteristics of particular subjects and ensure natural instance/scene interactions. We formalize this overlooked yet critical editing paradigm as "Get-In-Video Editing", where users provide reference images to precisely specify visual elements they wish to incorporate into videos. Addressing this task's dual challenges, severe training data scarcity and technical challenges in maintaining spatiotemporal coherence, we introduce three key contributions. First, we develop GetIn-1M dataset created through our automated Recognize-Track-Erase pipeline, which sequentially performs video captioning, salient instance identification, object detection, temporal tracking, and instance removal to generate high-quality video editing pairs with comprehensive annotations (reference image, tracking mask, instance prompt). Second, we present GetInVideo, a novel end-to-end framework that leverages a diffusion transformer architecture with 3D full attention to process reference images, condition videos, and masks simultaneously, maintaining temporal coherence, preserving visual identity, and ensuring natural scene interactions when integrating reference objects into videos. Finally, we establish GetInBench, the first comprehensive benchmark for Get-In-Video Editing scenario, demonstrating our approach's superior performance through extensive evaluations. Our work enables accessible, high-quality incorporation of specific real-world subjects into videos, significantly advancing personalized video editing capabilities.

==> sec/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure*}[t]
    \centering
    % \vspace{-0.3cm}
    \includegraphics[width=\textwidth]{figs/model_arch.pdf}
    %\vspace{-0.7cm}
    \caption{
    \textbf{The model architecture of \modelName}. 
    }
    \label{fig:model_arch}
    \vspace{-0.3cm}
\end{figure*}


Video editing has become increasingly important in various applications, including film production, social media content creation, and virtual reality experiences. Traditional video editing approaches often require extensive manual effort and professional expertise, limiting accessibility for average users~\cite{rana2021deepremaster, leake2017computational}. Recent advancements in AI-driven editing tools have made significant progress in automating various aspects of video manipulation, ranging from text-guided editing~\cite{bar2022text2live, kawar2023imagic, hong2022depth, wang2023videocomposer} to motion transfer and style adaptation.


However, existing methods predominantly rely on text prompts or predefined operations, which have inherent limitations when users want to communicate specific visual details. This limitation becomes particularly evident in an important yet underexplored scenario: when users need to incorporate specific real-world instances (such as a particular person, pet, or object) into a video. In such cases, textual descriptions fundamentally fall short of conveying the unique visual characteristics that define these subjects \cite{yang2023paint, gal2022image}. For example, when someone wishes to insert their friend or pet into a video, language alone cannot accurately capture the distinctive appearance features that make that individual recognizable.


We define this overlooked yet critical task as "\editingTask," where users provide reference images to precisely specify visual elements they wish to incorporate into videos. 

This approach faces two significant challenges. First, there is a severe scarcity of training data that pairs reference images with appropriately edited videos. 

Second, technical implementation demands that inserted objects be coherently embedded within the video context, exhibiting natural motion and plausible interactions with existing scene elements \cite{liu2023video, blattmann2023stable}. These requirements necessitate strong temporal consistency capabilities as the model must adapt the reference subject to varying poses, lighting conditions, and perspectives throughout the video sequence. 

To address these challenges:

we introduce \textbf{\datasetName} dataset, a million-scale dataset created through our automated Recognize-Track-Erase pipeline. This comprehensive pipeline integrates multiple state-of-the-art components: vision-language models for precise object identification and contextual video captioning, Ground-DINO for reliable instance detection, SAM2 for accurate temporal instance tracking, and ProPainter for clean instance removal. The resulting quintuple training samples—\textit{\{prompt, reference image, tracking mask, condition video (object-removed as input), target video (original)\}}—provide high-quality alignment between textual descriptions, visual contexts, and tracked object masks, effectively overcoming the data scarcity challenge while ensuring training data integrity.

% TODO[huangzp]: rewrite this paragraph
% TODO[huangzp]: rename the framework
Based on our large-scale dataset, we develop \textbf{\modelName}, a novel end-to-end framework that seamlessly integrates reference objects into target videos. Our approach addresses the technical challenges through three key consistency mechanisms: maintaining temporal coherence across video frames, preserving the visual identity of reference objects, and ensuring natural physical interactions with the original scene elements. This three-pronged consistency strategy enables our model to adapt reference objects to diverse poses, lighting conditions, and perspectives while maintaining realistic video dynamics.

To enable systematic evaluation, we introduce \textbf{\benchmarkName}, the first comprehensive benchmark specifically designed for reference-guided video object addition. This benchmark supports both qualitative and quantitative assessment through carefully curated test cases featuring both single-object and multi-object reference scenarios. Through extensive experimentation, \modelName demonstrates exceptional performance on this benchmark, outperforming existing approaches in visual quality and achieving significant quantitative advantages across multiple evaluation metrics.



Our principal contributions are as follows:
\begin{itemize}
\item We formalize \editingTask as a new editing scenario, addressing the fundamental limitations of previous approaches for incorporating specific real-world instances into videos.

\item We introduce \datasetName, a large-scale dataset specifically constructed for this task, containing 1 million video editing pairs with comprehensive textual annotations and reference images.

\item We develop \modelName, the first end-to-end model that effectively solves this challenging problem by maintaining temporal coherence, visual identity preservation, and natural scene interactions.

\item We establish \benchmarkName, the first comprehensive benchmark for this editing scenario, and demonstrate our approach's superior performance through extensive qualitative and quantitative evaluations.
\end{itemize}






==> sec/1_introduction_bak.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure*}[t]
    \centering
    % \vspace{-0.3cm}
    \includegraphics[width=\textwidth]{figs/model_arch.pdf}
    %\vspace{-0.7cm}
    \caption{
    \textbf{The model architecture of Get In Video}. 
    }
    \label{fig:model_arch}
    \vspace{-0.3cm}
\end{figure*}

The rise of diffusion models has revolutionized visual content generation, 
first catalyzing breakthroughs in text-to-image synthesis with commercial-grade outputs, 
and more recently propelling text-to-video systems to produce realistic, 
physics-compliant videos of remarkable visual quality. 
As controllability becomes increasingly crucial in generative tasks, 
researchers have explored injecting conditional signals like poses, 
edge maps, 
and depth maps into the generation process. 
This evolution highlights a critical industrial demand in film production: 
seamlessly integrating new objects into existing videos while maintaining both object consistency across frames and natural interactions with the original scene. 
Traditional solutions rely on labor-intensive post-production workflows, 
but the ascendancy of visual generative models raises an intriguing question: 
Can we develop an end-to-end framework for video object insertion?

Prior attempts focused primarily on image editing, 
yet video poses distinct challenges. 
First, 
data acquisition proves fundamentally difficult—existing video datasets rarely contain parallel sequences with and without specific environmental changes, 
necessitating systematic pipelines to synthesize training pairs. 
Second, 
computational demands escalate exponentially:
video models inherently require larger parameter spaces than image models, 
while frame-wise processing multiplies token counts. 
Conventional conditioning methods further exacerbate this burden through auxiliary network modules, 
rendering training or fine-tuning prohibitively expensive.

To address these challenges, 
we present \textbf{Get in Video}, 
a novel end-to-end framework that injects objects from reference images into video sequences while preserving threefold consistency: 
temporal coherence of the modified video, 
visual identity of the inserted object, 
and natural physical interactions with the original scene. 
For model training, 
we introduce \textbf{BrushVid-1M},
a million-scale dataset constructed through our automated Recognize-Track-Erase pipeline. 
Leveraging vision-language models for object identification and scene captioning, 
SAM2 for temporal mask generation, 
and ProPainter for object removal, 
we synthesize quintuple training samples \textit{\{prompt, 
reference image, 
mask image, 
condition video (object-removed), 
target video (original)\}}. 
This process ensures high-quality alignment between textual descriptions, visual contexts, and object masks.
To enable quantitative evaluation of generated results, 
we present \textbf{Get In Bench} – the first benchmark for reference image-based video object addition, 
designed for both qualitative and quantitative assessment of synthesized video quality. 
Notably, 
Get In Bench incorporates test cases containing both single-object and multi-object reference video generation, 
specifically designed to evaluate models' capability in handling multi-image reference scenarios. 
Our proposed Get In Video demonstrates superior performance on Get In Bench,
achieving not only the best visual quality in qualitative experiments but also establishing significant quantitative superiority through rigorous metric evaluation.

Our principal contributions are fivefold:
\begin{itemize}
\item We pioneer the task of reference-guided video object insertion, 
addressing a critical industrial need.

\item We propose Get In Video, 
the first end-to-end model for adding objects to videos based on reference images, 
and achieve state-of-the-art performance on video object addition.

\item We propose BrushVid, the first large-scale dataset for this task, provides 1 million video pairs with textual annotations.

\item We propose Get In Bench, the first benchmark for reference image-based video object addition.

\item Our framework demonstrates significant potential for streamlining professional video production pipelines.
\end{itemize}

==> sec/2_related_work.tex <==
\section{Related Work}
\label{sec:related_work}


==> sec/3_method.tex <==
\section{Method}
\label{sec:method}

In this section,
we introduce our Get In Video (GIV), 
the first generative model for adding objects to videos based on reference images. 
We first review the preliminaries of text-to-video diffusion model in Section 3.1, 
introduce the model architecture and training method of GIV in Section 3.2, 
and in Section 3.4, 
we introduce our proposed reference image video generation dataset BrushVid and its construction.

\subsection{Text-to-Video Diffusion Model}
\label{subsec:t2v_diffusion}

The diffusion model is designed to learn a data distribution by gradually denoising a normally-
distributed variable. 
It has been widely used for video generation.
Text-to-Video (T2V) diffusion model usually uses 3D-VAE encoder to compress the image or video $x$ into $z$ in latent space as $z_{0}=Encoder(x)$, 
$z_{0}\in R^{f\times c \times h \times w}$, 
$x\in R^{F\times 3 \times H \times W}$,
which $F$, $H$ and $W$ refer to the number of frames, height and width of image or video ($F=1$ in image).
$f$, $c$, $h$ and $w$ represent the shape of feature after 3D-VAE compression.
In GIV, $f=\lceil \frac{F-1}{4} \rceil+1$, $c=16$, $h=\frac{H}{8}$ and $w=\frac{W}{8}$.
In the forward diffusion process, 
one should add gaussian noise $\epsilon \sim \mathcal{N} \left( 0, I \right)$ on the input $z_{0}$,
in order to generate the noisy input $z_{t}$ at each timestep,
\begin{equation}
z_{t}=\sqrt{\overline{\alpha}_{t}}z_{0}+\sqrt{1-\overline{\alpha}_{t}}\epsilon
\label{eq:zt}
\end{equation}
where $t = 1, 2, \cdots , T$, 
and $T$ is the total number of timesteps in the forward process.
$\overline{\alpha}_{t}$ is a parameter related to $t$.
When $t$ approaches $T$, 
$\overline{\alpha}_{t}$ approaches $0$.
The training goal is to minimize the loss for denoising,
\begin{equation}
\mathcal{L}=\mathbf{E}_{z_{0},c,\epsilon,t} \left[ \|\epsilon - \epsilon_{\Theta} \left(z_{t},t,c \right) \|^{2}_{2} \right],~~ t \in [1,~T]
\label{eq:diff_loss}
\end{equation}
where $\epsilon_{\Theta}$ is the output of neural network with model parameters $\Theta$, and $c$ indicates the additional condition.

\subsection{Get In Video}
\label{subsec:giv}

As shown in Fig. \ref{fig:model_arch},
our model Get In Video (GIV) can accept four conditions include prompt, 
reference images, 
mask image and unedited video as condition video simultaneously as input.
In order to be able to input the unedited original video as  condition video for our GIV, 
we expand the number of input channels $c$ ($c=16$ in GIV) of the original input layer of the model to $2c$,
and used zero initialization for the parameters in the expanded channels to ensure that the input distribution of the T2V model would not be affected.
During training,
we input the condition video $x_{cond}$ and target video $x_{target}$ into 3D-VAE and get the compression latent $z_{cond}$ and $z_{target_0}$.
Following eq. \ref{eq:zt}, we add gaussian noise $\epsilon \sim \mathcal{N} \left( 0, I \right)$ on $z_{target_0}$,
\begin{equation}
z_{target_t}=\sqrt{\overline{\alpha}_{t}}z_{target_0}+\sqrt{1-\overline{\alpha}_{t}}\epsilon
\label{eq:ztarget}
\end{equation}
Then we concat $z_{cond}$ and $z_{target_t}$ in the feature dimension to get $z_{video_t}$,
\begin{equation}
z_{video_t}=\texttt{concat([}z_{target_t} \texttt{,} z_{cond} \texttt{],dim=1)}
\label{eq:zvideo}
\end{equation}
which $z_{video_t}\in R^{f\times 2c \times h \times w}$.
Likewise, 
we send all the reference pictures $x_{ref}=[x_{ref_{0}}, x_{ref_{1}}, ...,x_{ref_{n-1}}]$ into 3D-VAE to obtain the latent 
$z_{ref}\in R^{n \times c \times h \times w}$,
where $n$ refers to the number of objects used for reference video generation.
And we perform spatial downsampling and channel dimension repeat operations on the mask $m\in R^{1\times 1\times H \times W}$  in sequence,
\begin{equation}
z_{mask}=\texttt{resize(}m\texttt{,(}w\texttt{,} h\texttt{))}\texttt{.repeat(}n\texttt{,}c\texttt{,1,1)}
\label{eq:zmask}
\end{equation}
which $z_{mask}\in R^{n\times c\times h\times w}$.
Then we concat $z_{ref}$ and $z_{mask}$ in channel dimension to get $z_{image}$,
\begin{equation}
z_{image}=\texttt{concat([}z_{ref} \texttt{,} z_{mask} \texttt{],dim=1)}
\label{eq:zimage}
\end{equation}
Next,
we concat the latent of $z_image$ and $z_{video_t}$ in the frame dimension to get the model input $z_{input_t}$,
\begin{equation}
z_{input_t} = \texttt{concat([} z_{ref}\texttt{,} z_{video_t} \texttt{],dim=0)}
\label{eq:zt_}
\end{equation}
which $z_{input_t}\in R^{\left( n+f \right) \times 2c \times h \times w}$.
This means that we use the first $n$ frames of the input video as reference pictures to participate in the generation.

Following previous works,
GIV inherits the most advanced diffusion transformer architecture with 3D full attention.
This demonstrates that in the GIV framework, 
all inputs and conditional information inherently interact through the attention mechanism without requiring supplementary modules, 
which enables effective inheritance of the original T2V pre-trained parameters with only minimal adjustments to the input layer's channel dimensions.
The architectural integrity ensures optimal preservation of pre-trained knowledge while achieving efficient multimodal integration.


\subsection{BrushVid-1M Dataset}
\label{subsec:brushvid}






==> sec/4_experiments_bak.tex <==
\section{Experiments}
\label{sec:exp}

\input{tabs/GIB_sota_comparison}


\begin{figure*}[t]
    \centering
    % \vspace{-0.3cm}
    \includegraphics[width=\textwidth]{figs/sota_compare.pdf}
    %\vspace{-0.7cm}
    \caption{
    \textbf{Visual comparison with the SOTA model.} 
    }
    \label{fig:sota_compare}
    % \vspace{-0.3cm}
\end{figure*}

\subsection{\benchmarkName}
\label{subsec:gib}

We propose the first benchmark \benchmarkName (GIB) for reference image-based video object addition, 
consisting of 100 test cases constructed using the same methodology as the BrushVid dataset. 
Each case comprises five key components: 
{condition video, 
reference images, 
prompt, 
mask, 
target video}. 
The benchmark framework incorporates five evaluation metrics to comprehensively assess video generation quality:
(1) Fréchet Inception Distance (FID) \cite{heusel2017gans} is measured using CLIP-ViT-Base-32 \cite{radford2021learning} as the feature extractor, quantifying the distribution discrepancy between generated video frames and their target counterparts;
(2) Fréchet Video Distance (FVD) adopts I3D as the feature extractor to measure temporal coherence and distribution differences across complete video sequences;
(3) CLIP Score between image pair (CLIP-I) employs CLIP-ViT-Base-32 to evaluate semantic similarity between generated videos and target videos at the conceptual level;
(4) DINO Score between image pair (DINO-I) utilizes DINOv2-Base to capture fine-grained visual similarities between generated and target videos through detailed feature analysis.
(5) CLIP Score between text-image pair (CLIP-T) leverages CLIP-ViT-Base-32 to assess the semantic alignment between generated videos and their corresponding text prompts.
This multi-dimensional evaluation system combines spatial-temporal analysis (FID/FVD) with semantic consistency metrics (CLIP-I/CLIP-T) and detailed visual matching (DINO-I), 
ensuring comprehensive assessment of both static frame quality and dynamic video characteristics.

\subsection{Implementation Details}
\label{subsec:imple}


\textbf{Training.}
We employ CogVideoX-T2V 2B as our text-to-video (T2V) pretrained model.
Following the methodology outlined in Sec. \ref{subsec:method_model}, 
we expand the input channels of the input layer from 16 to 32,
with newly added channels being zero-initialized. 
Our experiments utilized the BrushVid dataset to train video models at 480×720 resolution. 
And we train 25-frame and 49-frame models respectively.
Two distinct model configurations were implemented: a 25-frame variant and an extended 49-frame architecture, each trained separately to evaluate temporal consistency under different sequence lengths.
To ensure temporal consistency in generated videos, 
we maintain a frame sampling interval of 1 throughout the training and inference process. 
We drop 20\% of prompts, 
20\% of reference images, 
and 50\% of masks during the training phase.
The optimization is performed using AdamW with hyperparameters $\beta_{1}=0.9$,
$\beta_{2}=0.95$, 
$\beta_{3}=0.98$, 
$\varepsilon=10^{-8}$, 
and weight decay of 1e-4. 
A consistent learning rate of 5e-6 is adopted for stable training. 
Full-parameter fine-tuning is conducted with mixed-precision training (bfloat16) and DeepSpeed ZeRO-2 optimization, 
executed on 8×A100 GPUs for 50,000 training steps.

\noindent\textbf{Inference.}
During the inference phase, 
we uniformly employ DDIM sampling with 50 denoising steps. 
For T2V models,
classifier-free guidance is systematically applied throughout the generation process, 
as formalized by the equation:
\begin{equation}
\begin{split}
\widetilde{\epsilon}_{\Theta}(z_t,t,c_{\text{t}})&= \epsilon_{\Theta}(z_t,t,\varnothing) \\
&+s_1(\epsilon_{\Theta}(z_t,t,c_{\text{t}})-\epsilon_{\Theta}(z_t,t,\varnothing))
\label{eq:cfg}
\end{split}
\end{equation}
where $c_{\text{t}}$ denotes the prompt condition and $s_1$ serves as a scaling parameter that modulates the control intensity of the prompt condition. 
During the inference process of our GIV, 
the conditional inputs comprise not only textual prompts but also reference images and corresponding masks, 
which collectively constitute the image-based condition $c_{\text{i}}$. Consequently, 
the classifier-free guidance sampling procedure in GIV can be formulated as the equation below:
\begin{equation}
\begin{split}
\widetilde{\epsilon}_{\Theta}(z_t,t,c_{\text{t}},c_{\text{i}})&= \epsilon_{\Theta}(z_t,t,\varnothing,\varnothing) \\
&+s_1(\epsilon_{\Theta}(z_t,t,c_{\text{t}},\varnothing)-\epsilon_{\Theta}(z_t,t,\varnothing,\varnothing)) \\
&+s_2(\epsilon_{\Theta}(z_t,t,c_{\text{t}},c_{\text{i}})-\epsilon_{\Theta}(z_t,t,c_{\text{t}},\varnothing))
\label{eq:icfg}
\end{split}
\end{equation}
where $c_{\text{i}}$ denotes the image condition and $s_2$ serves as a scaling parameter that modulates the control intensity of the image condition. 
We set $s_1=6$,$s_2=1.5$ during inference.

\subsection{Comparison with state-of-the-art}
\label{subsec:sota}

\textbf{Quantitative comparison.}
Tab. \ref{tab:gib_sota} presents a comprehensive comparison between our GIV framework and three representative methods: 
the renowned end-to-end image editing model InstructPix2Pix,
the reference-based image editing model Paint by Example, 
and the previous state-of-the-art video editing approach AnyV2V. 
The evaluation on the GIB benchmark demonstrates that GIV-generated videos achieve optimal performance across multiple critical metrics. 
% Notably, our framework exhibits superior distribution consistency with source videos while maintaining exceptional alignment with textual prompts and preserving semantic coherence through temporal sequences. 
These results comprehensively demonstrate GIV's superiority as the first end-to-end video editing framework capable of executing precise reference image-guided modifications while maintaining temporal stability and content fidelity.


\noindent\textbf{Qualitative comparison.}
As demonstrated in Fig. \ref{fig:sota_compare},
our GIV framework achieves superior performance in detail preservation and object insertion. 
Unlike previous methods, 
GIV not only maintains remarkable fidelity to the original video content but also seamlessly integrates reference objects into specified mask regions with pixel-level precision. 

\subsection{Ablation Study}
\label{subsec:abla}

\textbf{Quantitative comparison}


\noindent\textbf{Qualitative comparison}


==> sec/5_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
